Adapting the Hypersphere Loss Function from Anomaly Detection to Anomaly Segmentation

We propose an incremental improvement to Fully Convolutional Data Description (FCDD), an adaptation of the one-class classification approach from anomaly detection to image anomaly segmentation (a.k.a. anomaly localization). We analyze its original loss function and propose a substitute that better resembles its predecessor, the Hypersphere Classifier (HSC). Both are compared on the MVTec Anomaly Detection Dataset (MVTec-AD) -- training images are flawless objects/textures and the goal is to segment unseen defects -- showing that consistent improvement is achieved by better designing the pixel-wise supervision.

==> figs/00-convergence.tex <==
% \begin{figure}
% \centering
% \includegraphics[width=120mm]{accv22.png} 
% \caption{
% The website of ACCV 2022 is at \url{https://www.accv2022.org}. 
% If images are copied from some source then provide the reference.
% Follow copyright rules as they apply. A caption ends with a full stop.}
% \label{fig:ACCV22}
% \end{figure}


\begin{figure}[tb]
\centering
%
\subfigure[Semi-supervised]{
\label{fig:convergence-ssup}
\includegraphics[width=\textwidth]{imgs/00-convergence-semi-supervised.png}
}
%
\hfill
%
\subfigure[Unsupervised]{
\label{fig:convergence-unsup}
\includegraphics[width=\textwidth]{imgs/00-convergence-unsupervised.png}
}
%
\caption{
The test \gls{auroc} was recorded at the end of each training epoch, then the mean value and the standard deviation were computed over the six seeds at each epoch.
Each plot corresponds to a combination of supervision setting and normal class, displaying the losses "per-batch average" and "per-image average" for comparison.
The mean curves (usually at the upper part of the graphs) are displayed in blue and their scale is the left vertical axis; the standard deviation curves (usually at the bottom part of the graphs) are displayed in red and their scale is the right vertical axis.
The results for "per-batch average" are displayed in as solid lines, and the results for "per-image average" are displayed as dashed lines.
}
\label{fig:convergence}
\end{figure}




==> figs/03-cd-diagram-auroc.tex <==
\begin{figure}[tb]
\centering
\includegraphics[width=60mm]{imgs/03-cd-diagram-auroc.png} 
\caption{
}
\label{fig:03-cd-diagram-auroc}
\end{figure}


==> figs/04-cd-diagram-avg-precision.tex <==
\begin{figure}[tb]
\centering
\includegraphics[width=60mm]{imgs/04-cd-diagram-avg-precision.png} 
\caption{
}
\label{fig:04-cd-diagram-avg-precision}
\end{figure}

